Continual Segment: Towards a Single, Unified and Accessible Continual Segmentation Model of 143 Whole-body Organs in CT Scans

Deep learning empowers the mainstream medical image segmentation methods. Nevertheless current deep segmentation approaches are not capable of efficiently and effectively adapting and updating the trained models when new incremental segmentation classes (along with new training datasets or not) are required to be added. In real clinical environment, it can be preferred that segmentation models could be dynamically extended to segment new organs/tumors without the (re-)access to previous training datasets due to obstacles of patient privacy and data storage. This process can be viewed as a continual semantic segmentation (CSS) problem, being understudied for multi-organ segmentation. In this work, we propose a new architectural CSS learning framework to learn a single deep segmentation model for segmenting a total of 143 whole-body organs. Using the encoder/decoder network structure, we demonstrate that a continually-trained then frozen encoder coupled with incrementally-added decoders can extract and preserve sufficiently representative image features for new classes to be subsequently and validly segmented. To maintain a single network model complexity, we trim each decoder progressively using neural architecture search and teacher-student based knowledge distillation. To incorporate with both healthy and pathological organs appearing in different datasets, a novel anomaly-aware and confidence learning module is proposed to merge the overlapped organ predictions, originated from different decoders. Trained and validated on 3D CT scans of 2500+ patients from four datasets, our single network can segment total 143 whole-body organs with very high accuracy, closely reaching the upper bound performance level by training four separate segmentation models (i.e., one model per dataset/task).

==> method_original.tex <==
%\subsection{Problem Formulation}
% \Ac{gs} is designed to continuously learn a single model on restrained data from sequential tasks, i.e., data from different tasks are not simultaneously available for learning, and data from the previous tasks might not be accessible when training future tasks. In a more challenging clinical practice, \ac{gs} needs to tackle both class-incremental and domain-incremental settings, especially when the dataset size, anatomy structure classes, and scanning sections vary throughout different tasks. Let $D=\{D_1, \dots, D_T\}$ denote a sequence of data. For the $t^{th}$ task $D_t=\{{x_i}^t, {y_i}^t\}_{i=1}^{n_t}$, let $x^t$ and $y^t$ denote the input image and the corresponding organ label of the $t^{th}$ task, \ac{gs} aims to train a single model s.t. the prediction map for voxel location, $j$, and output class $c^t$:
% \begin{align}
%     \hat{y}^t(j) &= f_d\left(y^t(j)=c^t|f_e\left(x^t; \theta_e^t\right); \theta_d^t\right), \\
%     \hat{y} &=\bigcup_{i=1}^{T}{\hat{y}^t}, \, t\in\{1, \dots, T\}
% \end{align}
% where $f_e$, $f_d$, $\theta_e$, and $\theta_d$ denote the CNN functions and the corresponding parameters for the encoding and decoding paths, respectively. The final prediction $\hat{y}$ is the union of all previous predictions. 


%Dazhou original: We aim to continuously learn a single model on restrained data from sequential tasks, i.e., data from different tasks are not simultaneously available for learning; data from the previous tasks might not be accessible when training future tasks. In a more challenging clinical practice, the model must tackle both class-incremental and domain-incremental settings, involving significant variations in the dataset size, anatomical structures, and scan \ac{fov} across different tasks. Let $D=\{D_1, \dots, D_T\}$ denote a sequence of data. For the $t^{th}$ task $D_t=\{{X_i}^t, {Y_i}^t\}_{i=1}^{n_t}$, let $X^t$ and $Y^t$ denote the input image and the corresponding organ label of the $t^{th}$ task, the prediction map for voxel location, $j$, and output class $C^t$:



% is not consistently defined -- some anatomical structures of classes in a particular downstream task might be marked/annotated as the background classes from other tasks/datasets. To mitigate these issues, we propose  


% 1) Unseen body parts can be found later, implying that \ac{ge}'s feature abstractions could have some representation limitations or restrictions at the current training step; 2)

% In addition, we need to gain a thorough understanding of another critical issue (that can be overlooked otherwise) 


% First, we need to gain a thorough understanding of two critical issues (that can be overlooked otherwise): 1) 




% Fortunately, medical imaging is in a much more confined domain, i.e., the human body is anatomically structured and composed of distinct body parts, which makes it possible to obtain a strong \ac{ge} even with limited or not-so-limited training data.

% However, we need to gain a thorough understanding of two critical issues (that can be overlooked otherwise) in whole-body organ segmentation model training, especially when dealing with 142 organs or classes collected from multiple large datasets. 1) Unseen body parts can be found later, implying that General Encoder's feature abstractions could have some representation limitations or restrictions at the current training step; 2) Background class is not consistently defined -- some anatomical structures of classes in a particular downstream task might be marked/annotated as the background classes from other tasks/datasets. %The network subsequently would emphasize the foreground classes~\cite{zhoubolei CAM} while making it hard to optimize those structures hidden in the fake background. "it is very unclear what you are trying to say here ....(got it)"
%\ac{fbkg} is not a good word, nobody really knows what fake background (conflict labels?) means ... it is not a scientifically defined word, thus your following few sentences .... not understandable!!

% \textcolor{red}{How do you solve these two issues???}

% The network thus would have false-positives predictions in unseen body parts

% To address these issues, we exploit body parts labels 

% introduce the \ac{fbkg} to the training process. We use \textit{upper lung tip}, \textit{lower lung tip}, \textit{lower spine} to separate the body into head \& neck, thorax, abdomen, hip \& thigh regions. Instead of training a nnUNet with a single anatomical structure segmentation head, we add another segmentation head for the \ac{fbkg} segmentation. Considering the \ac{fbkg} consists of distinct anatomical features, making segmentation straightforward. We segment \ac{fbkg} using the PSNN~\cite{dakai gtv paper} decoding architecture, a super-lightweight decoder head with accumulated side outputs. Depicted in \Fig{xxx}, a strong \ac{ge} can be obtained using a comprehensive dataset with \ac{fbkg}, e.g., TotalSegmentator dataset + \ac{fbkg} segmentation head. 


% Processing \ac{ge} training, we start with complementing the training dataset with \ac{fbkg} labels. 

% We use the body parts label  head \& neck, thorax, abdomen, hip \& thigh. 

% Concerning some of the classes in $y_t$ that could overlap between tasks, 

% Most leading approaches~\cite{xxxx} 

% In order to  straightforward solution is to train separate models 


% In a more challenging clinical practice, data size and class number vary significantly throughout different tasks. We might also encounter a scenario when a dedicated dataset (usually with tumors) is proposed to update existing organs.  



% the \ac{ge} extracts features for each downstream task, 



 % which involves three components to stratify 
% The general idea of general-encoder + multi-head decoding paths


% \textcolor{red}{\Fig{xxx}} demonstrates average segmentation performance from using weaker to stronger pre-trained \ac{ge}. 





% Next, we validate the key element \ac{ge}, which holds our main assumption of the framework.

% Anatomy structure labeling is expensive and expertise-demanding. 

% We denote those foreground body parts as fake-background labels. 

% Similar to pioneer work~\cite{amazon...CIL}, we first analyze if we need to optimize 


% We first analyze 

% the entire pre-trained \ac{ge} using novel data. \textcolor{red}{\Fig{xxx} or \Tab{xxx}} demonstrates average segmentation performance from using weaker to stronger pre-trained \ac{ge}, 

% the new organs in the head \& neck and thoracic regions  

% training a nnUNet segmentation model using the TotalSegmentator dataset~\cite{wasserthal2022totalsegmentator}, which covers the majority parts of the human body





% when there is a set of anatomical structures, e.g., bone, muscle, organ, soft tissue, and how many structures would facilitate the novel class optimization. Unlike natural images, where objects hold various sizes, shapes, and inner contexts in diverse scenarios, medical imaging is much more confined, i.e., the human body is anatomically structured and composed of distinct body parts. We begin with TotalSegmentator~\cite{wasserthal2022totalsegmentator} as our starting point


% This intuitively gives ways to assume that we could use relatively less a \ac{ge} to learn sufficient features for the downstream tasks. 


% when there is a set of anatomical structures, e.g., bone, muscle, organ, soft tissue, and how many structures would facilitate the novel class optimization. Unlike natural images, where objects hold various sizes, shapes, and inner contexts in diverse scenarios, medical imaging is much more confined, i.e., the human body is anatomically structured and composed of distinct body parts. We begin with TotalSegmentator~\cite{wasserthal2022totalsegmentator} as our starting point


% This intuitively gives ways to assume that we could use relatively less a \ac{ge} to learn sufficient features for the downstream tasks. 


% organ is an anatomically distinct structure of the body 

% Detailed general encoding for each task + (maybe) body parts/disease target 


% But the decoding paths accumulated when more tasks are added, requiring trim of much efficient and light-weight decoders. 

%Stratified Decoding
\subsection{Decoder Optimization}
Equipped with the shared and frozen \ac{ge} from Sec.~\ref{sec:ge}, \ac{gs} gradually obtains scalable segmentation model capacities by adding and training separate decoding heads for the added tasks or datasets (of the lung, esophageal and head-and-neck cancer patients) where each task-specific decoding path can be independently optimized. Considering the significant variations in anatomical structures and body parts for different tasks, it is likely that each task would benefit from decoding architectures tailored to their needs. However, as more tasks are incrementally included, the overall \ac{gs} size escalates and might cause the parameter explosion, s.t., fewer tasks could be included in \ac{gs} when the GPU RAM is limited. For each decoding path, we propose a two-step decoder optimization scheme by 1) automatically searching decoder architecture for optimal performance; 2) progressively trimming convolutional blocks for a compressed decoder head. In the following, we first discuss performance optimization in detail. 



% In this section, we perform network architectural optimization 

% Before obtaining the unified prediction, all  


% However, as more tasks are incrementally included, the overall \ac{gs} size escalated, eventually causing parameter explosion given limit-sized GPU RAM. Not to mention the extended inference time. 


% The decoding paths accumulate the complexity when more datasets are incrementally added and trained. To achieve the final semantically consistent segmentation output in Sec. \ref{sec:merging}, we would need to combine and merge the segmentation output class spaces generated from all decoding heads to the final total 142 organs/classes. \textcolor{red}{Before the segmentation decoder label merging, in this section we perform network architectural optimization and knowledge distillation on each decoder to improve the segmentation accuracy, efficiency and generalizability in the following two steps....Each important and contributing technical component needs to be adequately motivated and clearly described.} %\textcolor{red}{\Fig{xxx}} illustrates our generalizability decoding. The first stratification dimension exploits NAS to search distinct network architectures for each task. The second dimension stratification uses block-wise teacher-student knowledge distillation frameworks to see if we could trim each decoder head even further with an acceptable performance drop. 

\noindent\textbf{Performance Optimization -- NAS.}
% We aim to optimize the segmentation performance by exploiting NAS to tailor the task-specific decoding path to its need.  
Let $\phi\left( \cdot; \omega_{x \times y \times z} \right)$ denote a composition function of consecutive operations: batch normalization, a rectified linear unit, and a convolution layer with an $x \times y \ times z$ dimension kernel. We search for a set of possible architectures involving: projection convolution $\phi\left( \cdot; \omega_{1 \times 1 \times 1} \right)$, 2D convolution $\phi\left( \cdot; \omega_{3 \times 3 \times 1} \right)$, pseudo-3D convolution $\phi\left( \phi\left( \cdot; \omega_{3 \times 3 \times 1} \right); \omega_{1 \times 1 \times 3} \right)$, and 3D convolution $\phi\left( \cdot; \omega_{3 \times 3 \times 3} \right)$. To simplify the searching process, we use only one type of convolutional kernel to build each decoding block. We relax the searching by assigning each category a weight. At the end of the search, we determine the network architecture of each block by choosing the $\phi$ corresponding to the largest weight value. 

Due to the search space including down-sized convolutional kernels (e.g., 2D vs. 3D), the decoder architecture might select lightweight convolutional kernels for optimal performance. However, using NAS cannot guarantee obtaining a compressed decoder head. Next, we introduce progressive trimming for decoder compression. 

% The default is on the nnUNet decoding path, of which architectures .  

% Considering the significant variations in anatomical structures and \ac{fov} of different tasks, it is likely that each task would benefit from decoding architectures tailored to their needs. To do this, we automatically search network architecture for each decoding head. Let $\phi\left( \cdot; \omega_{x \times y \times z} \right)$ denote a composition function of consecutive operations: batch normalization, a rectified linear unit, and a convolution layer with an $x \times y \ times z$ dimension kernel. We search for a set of possible architectures involving: projection convolution $\phi\left( \cdot; \omega_{1 \times 1 \times 1} \right)$, 2D convolution $\phi\left( \cdot; \omega_{3 \times 3 \times 1} \right)$, pseudo-3D convolution $\phi\left( \phi\left( \cdot; \omega_{3 \times 3 \times 1} \right); \omega_{1 \times 1 \times 3} \right)$, and 3D convolution $\phi\left( \cdot; \omega_{3 \times 3 \times 3} \right)$. To simplify the searching process, we use only one type of convolutional kernel to build each decoding block. We relax the searching by assigning each category a weight. At the end of the search, we determine the network architecture of each block by choosing the $\phi$ corresponding to the largest weight value. 

\noindent\textbf{Size Optimization -- Progressive Trimming.}
When adding more tasks, the \ac{gs} might suffer a parameter explosion issue, which limits the maximum number of tasks  that could be accommodated and prolongs the per-task inference time. We propose a progressive trimming scheme to compress each decoding head under an acceptable performance drop, e.g., relative $1\%$ -- from $80.0\%$ to $79.2\%$.

Before starting the trimming process, we first train the NAS searched decoder head (from the previous step) to its optimal performance, then we freeze the trained decoder head and use it as the teacher decoder. The teacher-student architecture-based compression framework~\cite{deng2020model} is adopted. We pair each teacher's convolutional block with a projection block (i.e., a convolutional block with projection layers), targeting to exploit the student blocks to replace the teacher blocks. The mean-square error loss is used to match the feature maps of the teacher block to the student block. To reduce the optimization difficulty, we first distill the deeper decoding blocks. Once the \ac{kd} training of the deeper block is saturated, we freeze the deeper student blocks and then progressively move to the shallower ones. 

% given the feature maps to both teacher and student blocks, 
%In an ideal case, the output activation maps of the teacher and student blocks are the same. We could expect the teacher block and the student block to generate the same segmentation predictions. However, in most cases, the output activation maps of the teacher and student blocks are not the same. The subtle differences would change the subsequent feature response of the shallower blocks, resulting in degenerated segmentation. We employ a simple yet effective approach to tackle this issue: After the initial \ac{kd} training of the student block is finished, we adopt a small learning rate (e.g., $10\times$ less) and finetune (e.g., 10 epochs) the shallower teacher blocks using the deeper student block's output feature maps. We then monitor the before-and-after performance drop. If the drop is less than relative $1\%$, we keep the deeper student block, otherwise, we restore the teacher blocks. To speed up the training process, block-wise side supervision is also used during finetuning. After we determined the trimmed architecture (with acceptable performance drop rates), we finetune the trimmed decoder head again using a smaller learning rate (e.g., $20\times$ less). In the following, we elaborate on the merging of predictions from all previous tasks. 

% Note that our teacher-student architecture design will allow the shallower 
% The progressive trim involves a block-wise teach-student \ac{kd} process and a progressive finetune process.  


% Specifically, we perform a block-wise teacher-student \ac{kd} scheme for knowledge distillation, targeting to exploit the convolutional block with the projection kernels to replace those with the searched kernels. The mean-square error loss is used to match the feature maps of the teacher block to the student block. To ease the optimization difficulty, we first distill the deeper decoding blocks, then to the shallower blocks. Once the \ac{kd} training of the deeper block is saturated, we freeze the deeper student blocks and move to the shallower ones. 

% As our goal is to replace the decoding block with the projection block, the shallower block will have to `choose' if to receive output feature maps from the deeper teacher blocks or those from the student block. This causes an input discrepancy issue, i.e., the input feature map differences might change the subsequent feature response and result in degenerated segmentation. We employ a simple yet effective approach to tackle this issue: Once the \ac{kd} of the student block is finished, we adopt a small learning rate (e.g., $0.1\times$) and finetune the shallower teacher block using the deeper student block's output feature maps. We monitor the before-and-after performance drop. If the drop is less than relative $1\%$, we keep the deeper student block, otherwise, we restore the teacher blocks. To speed up the training process, block-wise side supervision is also used during training. 

% While tailoring the decoding head for each task could down-size the network, using NAS \textbf{\textit{cannot}} guarantee (even involving smaller convolution kernel search) to obtain a lightweight decoding head. Because NAS, by its nature, is to find the optimal architecture with the best performance. We aim to trim each decoding head under an acceptable performance drop, e.g., relative $1\%$ -- from $80.0\%$ to $79.2\%$. We perform a block-wise teacher-student \ac{kd} scheme for trimming, targeting to exploit the convolutional block with the projection kernels to replace those with the searched kernels.  We use the mean-square error loss to match the feature maps of the teacher block to the student block. To ease the optimization difficulty, we first distill the deeper decoding blocks, then to the shallower blocks. Once the \ac{kd} training of the deeper block is saturated, we freeze the student deeper blocks and move to the shallower ones. 

% As our goal is to replace the decoding block with the projection block, yet the shallower block will have to `choose' between the output feature maps from the deeper teacher blocks and from the student block. This causes an input discrepancy issue, i.e., the input feature map differences might change the subsequent feature response and result in degenerated segmentation. We employ a simple yet effective approach to tackle this issue: Once the \ac{kd} of the student block is finished, we adopt a small learning rate (e.g., $0.1\times$) and finetune the shallower teacher block using the deeper student block's output feature maps. We monitor the before-and-after performance drop. If the drop is less than relative $1\%$, we keep the deeper student block, otherwise, we restore the teacher blocks. To speed up the training process, block-wise side supervision is also used during training. 



% we might encounter an input discrepancy issue, i.e., the shallower block will receive two types  


% multi-head decoding path + decoding path compression

% processing NAS

% processing teacher-student knowledge distillation

\subsection{Anomaly-aware Decoder Merging} 
\label{sec:merging}
% Denoted in Eq.~(\ref{eq:gs}), the final output of the \ac{gs} is a unified prediction of all tasks.
To achieve the final semantically consistent segmentation output, we would need to combine and merge the segmentation output class spaces generated from all decoding heads to the final total of 142 organs/classes. In a more challenging clinical practice, medical images might contain anomaly tissues, e.g., tumors. Therefore, in addition to the existing segmentation tasks, we supplement the \ac{gs} with a PSNN-based tumor segmentation head to identify distinct tumors $\hat{Y}^{\epsilon}$. The average tumor size $p^{\epsilon}$ is calculated using the tumor dataset. Let $g(\cdot)$ denote a 3D zero mean Gaussian kernel of a given standard deviation. To avoid possible tumor false positives, we further smooth the $\hat{Y}^{\epsilon}$ using a Gaussian filter  $g(p^{\epsilon})$. 

Due to different organs may share similar textures, another challenging but overlooked problem in label merging is that the trained model might predict high-confident false positives in unseen body parts, e.g., the head \& neck model predicts parotid gland near the liver region. To avoid out-of-body part false positives, for each task, we also calculate 1) the average patient-wise \ac{fov} size $p^{t}$ -- the average size of the bounding box of all labeled classes; 2) the majority voted body part -- the body parts with the most overlapped \ac{fov}. Let $\hat{Y}^t_{\beta}$ denote the predicted body parts from Sec.~\ref{sec:ge}. We remove the falsely predicted body parts by smoothing $\hat{Y}^t_{\beta}$ with a Gaussian filter  $g(p^{t})$. 


\begin{algorithm}[ht!]
 \caption{Abnormality-sensitive merging}\label{alg:merging}
 \KwIn{$\hat{Y}^t$, $\hat{Y}^{\epsilon}$, $\hat{Y}^t_{\beta}$, $p^{\epsilon}$,  $p^{t}$}
 \KwOut{$\hat{\mathbf{Y}}$}
  \textbf{Initialize:} $\hat{\mathbf{Y}} \gets \emptyset$, $\hat{Y}^{\epsilon} \gets g\left(p^{\epsilon}\right) \otimes \hat{Y}^{\epsilon}$\\
  \For{$t \gets 1, \dots, T$}{
     $\hat{Y}^{t}_{\beta} \gets \hat{Y}^{t}_{\beta} \otimes g\left(p^{t}\right) $\\
     $M^{t} \gets \dfrac{1}{2}\left(J - \hat{Y}^{\epsilon} + \hat{Y}^{\epsilon} \odot \hat{Y}^t_{\beta}\right)$\\
     $H^t \gets - \left(M^{t} \odot \hat{Y}^t\right) \log\left(M^{t} \odot \hat{Y}^t\right)$ \\
     % $\mathbf{H} \gets \mathbf{H} \cup H^t$
  }
  $\mathbf{H}(j) \gets \bigcup_{\forall \hat{Y}(j)^t \neq 0}{H^t(j)}, t\in\{1, \dots, T\}$ \\
  $\hat{\mathbf{Y}}(j) \gets \hat{Y}^{\argmin(\mathbf{H}(j))}(j)$
\end{algorithm}

We present a whole picture of the merging procedure in Algorithm~\ref{alg:merging}. Let $\odot$ denote the element-wise multiplication and $J$ denote the matrix of ones, the weighting map $M^t$ is calculated, i.e., when only $Y^{\epsilon} \rightarrow 0$ and $Y^{t}_{\beta} \rightarrow 1$ s.t. the $M^t \rightarrow 0$, whereas $M^t \rightarrow 0.5$ for the rest states. Paring $M^t$ with each corresponding $\hat{Y}^t$, we use the entropy function to measure confidence. For each voxel, we collect a set $\mathbf{H}(j)$, for all $\hat{Y}(j)^t \neq 0$. The final output class $\hat{\mathbf{Y}}(j)$ is determined using the prediction $\hat{Y}^t(j)$, of which with the smallest $H^t(j)$.
% making the \ac{gs} unable to tell if the prediction of one head is more confident than the one of another head. 

% In addition to the existing segmentation tasks, we supplement the \ac{gs} with a PSNN-based tumor segmentation head to identify distinct tumors $\hat{Y}^{\epsilon}$. The average tumor size $p^{\epsilon}$ is calculated using the tumor dataset. 




% Concerning variations in body parts, anatomical structures, label overlapping, and possible existing tumors, we propose an anomaly-aware merging scheme.

% Denoted in Eq.~(\ref{eq:gs}), the final output of the \ac{gs} is a unified prediction of all tasks. In addition to the existing segmentation tasks, we supplement the \ac{gs} with a PSNN-based tumor segmentation head to identify distinct tumors $\hat{Y}^{\epsilon}$. The average tumor size $p^{\epsilon}$ is calculated using the tumor dataset. To avoid possible out-of-\ac{fov} false positives, for each task, we also calculate 1) the average \ac{fov} size $p^{t}$; 2) the majority voted body part. Using the predicted \ac{fbkg}, we obtain the \ac{fov} prediction $\hat{Y}^t_{\beta}$. Let $g(\cdot)$ denote a 3D zero mean Gaussian kernel of a given standard deviation. For each task, we first smooth both $\hat{Y}^t_{\beta}$ and $\hat{Y}^{\epsilon}$ using Eq.~(\ref{eq:smooth}), where $\otimes$ denotes the matrix convolution. Let $\odot$ denote the element-wise multiplication and $J$ denote the matrix of ones, the weighting map $M^t$ is calculated using Eq.~(\ref{eq:weighting}), i.e., when only $M^{\epsilon} \rightarrow 0$ and $M^{t}_{\beta} \rightarrow 1$ s.t. the $M^t \rightarrow 0$, whereas $M^t \rightarrow 0.5$ for the rest states. Paring $M^t$ with each corresponding $\hat{Y}^t$, we use the entropy function Eq.~(\ref{eq:confidence}) to measure confidence.

% % Next, we employ the binary entropy function to calculate the prediction confidence. 

% % and $\odot$  

% % and element-wise multiplication, respectively. The voxel-wise confidence is obtained using Eq.~(\ref{eq:confidence}).
% \begin{align}
% M^{\epsilon} &= \hat{Y}^{\epsilon} \otimes g\left(p^{\epsilon}\right) , M^{t}_{\beta} = \hat{Y}^{t}_{\beta} \otimes g\left(p^{t}\right) ,\label{eq:smooth}\\ 
% % M^{t}_{\beta} &= \hat{Y}^{\epsilon} \otimes g\left(p^{\epsilon}_{size}\right), \label{eq:mask_bodypart}  \\
% M^{t} &= \frac{1}{2} \left(J - M^{\epsilon} + M^{\epsilon} \odot M^t_{\beta}\right)\label{eq:weighting} \\
% H^t &= - \left(M^{t} \odot \hat{Y}^t\right) \log\left(M^{t} \odot \hat{Y}^t\right), \label{eq:confidence}\\
% \mathbf{H}(j) &= \bigcup_{\forall \hat{Y}(j)^t \neq 0}{H^t(j)}, t\in\{1, \dots, T\},\\
% \hat{\mathbf{Y}}(j) &= \hat{Y}^{\argmin(\mathbf{H}(j))}(j) \label{eq:final}.
% \end{align}
% For each voxel, we collect a set $\mathbf{H}(j)$, for all $\hat{Y}(j)^t \neq 0$. Depicted in Eq.~(\ref{eq:final}), the final output class $\hat{\mathbf{Y}}(j)$ is determined using the prediction $\hat{Y}^t(j)$, of which with the smallest $H^t(j)$.

% confident based merging -- weighting map * p log (p)

% tumor detection/segmentation module + p.log(p)-wise merging

% tumor detection -- lung + eso tumors

% abnormality-sensitive voxel-wise merging

% confidence-wise merging

==> tables/tab_eso_organ.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table}
\centering
\caption{Mean and standard deviation of DSC (\%, $\uparrow$), HD95 (mm, $\downarrow$) and ASD (mm, $\downarrow$) of esophagus in EsoOrgan of upper bound model and our final model.}
\label{tab:eso_organ}
\vspace{1em}
\resizebox{0.88\columnwidth}{!}{%
\begin{tabular}{@{}ll|lll@{}}
\toprule
\multicolumn{2}{l|}{\multirow{2}{*}{\textbf{Models}}} & \multicolumn{3}{c}{\textbf{EsoOrgan --- Eso}}  \\ \cmidrule(l){3-5} 
\multicolumn{2}{l|}{}                                 & \textbf{Dice}  & \textbf{HD95} & \textbf{ASD}  \\ \midrule
\multicolumn{2}{l|}{\textbf{Upper Bound}}             & 87.15$\pm$6.76 & 4.44$\pm$5.84 & 0.98$\pm$1.63 \\ \midrule
\multicolumn{2}{l|}{\textbf{Ours}}                    & 86.94$\pm$6.96 & 5.04$\pm$6.37 & 1.11$\pm$1.71 \\ \bottomrule
\end{tabular}%
}
\end{table}

==> tables/tab_step_dsc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}
\caption{Mean DSC of each comparison method over all learned classes at each step of two CSS orders. (Fig. \ref{M-fig:step_all}, the left one)} %}
\label{tab:step_dsc}
\resizebox{\columnwidth}{!}{%
%\scalebox{0.88}{
\begin{tabular}{l|rrrr}
\hline
\textbf{Order A}     & \multicolumn{1}{l}{\textbf{Step 0 (103)}} & \multicolumn{1}{l}{\textbf{Step 1 (130)}} & \multicolumn{1}{l}{\textbf{Step 2 (143)}} & \multicolumn{1}{l}{\textbf{Step 3 (143)}} \\ \hline
\textbf{MiB~\cite{cermelli2020modeling}}         & 93.24                                     & 50.56                                     & 20.86                                     & 8.51                                      \\
\textbf{$\textbf{ILT}^\dagger$~\cite{michieli2019incremental}} & 93.24                                     & 54.40                                     & 23.08                                     & 11.99                                     \\
\textbf{PLOP~\cite{douillard2021plop}}        & 93.24                                     & 62.40                                     & 45.10                                     & 39.01                                     \\
\textbf{LISMO~\cite{liu2022learning}}       & 93.24                                     & 57.74                                     & 22.86                                     & 12.11                                     \\
\textbf{Ours}        & 92.98                                     & 88.27                                     & 87.88                                     & 87.87                                     \\ \hline\hline
\textbf{Order B}     & \multicolumn{1}{l}{\textbf{Step 0 (103)}} & \multicolumn{1}{l}{\textbf{Step 1 (116)}} & \multicolumn{1}{l}{\textbf{Step 2 (143)}} & \multicolumn{1}{l}{\textbf{Step 3 (143)}} \\ \hline
\textbf{MiB~\cite{cermelli2020modeling}}         & 93.24                                     & 29.42                                     & 23.85                                     & 20.20                                     \\
\textbf{$\textbf{ILT}^\dagger$~\cite{michieli2019incremental}} & 93.24                                     & 29.09                                     & 26.13                                     & 22.44                                     \\
\textbf{PLOP~\cite{douillard2021plop}}        & 93.24                                     & 49.70                                     & 38.99                                     & 36.63                                     \\
\textbf{LISMO~\cite{liu2022learning}}       & 93.24                                     & 31.51                                     & 26.84                                     & 23.09                                     \\
\textbf{Ours}        & 92.98                                     & 91.27                                     & 87.88                                     & 87.87                                     \\ \hline
\end{tabular}%
}
\end{table}
